The Simons Observatory Large Aperture Telescope Receiver

The Simons Observatory (SO) Large Aperture Telescope Receiver (LATR) will be coupled to the Large Aperture Telescope located at an elevation of 5,200 m on Cerro Toco in Chile. The resulting instrument will produce arcminute-resolution millimeter-wave maps of half the sky with unprecedented precision. The LATR is the largest cryogenic millimeter-wave camera built to date with a diameter of 2.4 m and a length of 2.6 m. It cools 1200 kg of material to 4 K and 200 kg to 100 mk, the operating temperature of the bolometric detectors with bands centered around 27, 39, 93, 145, 225, and 280 GHz. Ultimately, the LATR will accommodate 13 40 cm diameter optics tubes, each with three detector wafers and a total of 62,000 detectors. The LATR design must simultaneously maintain the optical alignment of the system, control stray light, provide cryogenic isolation, limit thermal gradients, and minimize the time to cool the system from room temperature to 100 mK. The interplay between these competing factors poses unique challenges. We discuss the trade studies involved with the design, the final optimization, the construction, and ultimate performance of the system.

==> LATR_cutaway.tex <==
%========================================================%
\begin{figure*}[t]
  \centerline{
    \includegraphics[width=\linewidth]
{figs/LATR_xsection.png}
}
  \caption{Cross section of the LATR with primary components labeled. The 300\,K stage, which is 2.7\,m in diameter and 2.4\,m long, is divided into two main cylindrical components, the front section and the back. To control the radiative load, there is both an 80\,K and 40\,K stage.  The 80\,K stage is cooled by two PT90 refrigerators, while the 40\,K and 4\,K stages are cooled by two PT420 refrigerators.  The 1\,K and 100\,mK stages are cooled by a dilution refrigerator (DR).  
    \label{fig:LATR_cutaway}}
\end{figure*}
%========================================================%
